Distributed Charging Coordination of Electric Trucks with Limited Charging Resources

Electric trucks usually need to charge their batteries during long-range delivery missions, and the charging times are often nontrivial. As charging resources are limited, waiting times for some trucks can be prolonged at certain stations. To facilitate the efficient operation of electric trucks, we propose a distributed charging coordination framework. Within the scheme, the charging stations provide waiting estimates to incoming trucks upon request and assign charging ports according to the first-come, first-served rule. Based on the updated information, the individual trucks compute where and how long to charge whenever approaching a charging station in order to complete their delivery missions timely and cost-effectively. We perform empirical studies for trucks traveling over the Swedish road network and compare our scheme with the one where charging plans are computed offline, assuming unlimited charging facilities. It is shown that the proposed scheme outperforms the offline approach at the expense of little communication overhead.

==> recycle.tex <==
\newpage
\section{Distributed Optimization and Coordination of Charging Strategy}\label{Section IV}

\subsection{Route Model}
\begin{figure}[t!]
     \centering
     \includegraphics[width=0.99\linewidth]{F1.jpg}
      \caption{The route model of every electric truck, where ramps are denoted by $r_k$ while charging stations are denoted by $S_k$, $k\!=\!1,\dots,N$.}
      \vspace{-10pt}
      \label{Fig.1}
   \end{figure}
Throughout this paper, we consider a simplified route model for every electric truck, as illustrated in Fig.~\ref{Fig.1}. Specifically, we assume that there is a pre-planned route between the origin $O$ and destination $D$ of each truck to fulfill a certain delivery task. Along this route, $N$ charging stations are available to visit with each charging station being represented as $S_k$, $k\!=\!1,\dots,N$. The number of charging ports at each local station is limited and denoted by $G_k$. Furthermore, we refer to the ramp in the route that leads to the shortest detour reaching the station $S_k$ as the ramp $r_k$. For ease of notation, the origin and destination of a trip are denoted by $r_0$ and $r_{N+1}$, respectively. 

Towards depicting the dynamics of each truck, we denote by $\tau_k$, $k\!=\!0,\dots,N$, the travel time needed by the truck to traverse its route segment connecting its ramp $r_k$ and $r_{k+1}$. In addition, the travel time to take a one-way detour between the ramp $r_k$ and the station $S_k$ is denoted as $d_k$. 

\subsection{Remaining Battery and Waiting Budget}
Trucks need to take care of their remaining batteries and waiting budgets (i.e., the total waiting time that a truck can use in its entire trip) by optimally making their charging strategies so that trucks are able to reach their destinations on time before running out of their batteries. The optimal charging strategy consists of the following two decisions: (i) whether to charge the truck at a station $S_k$; and (ii) how long to charge the truck if deciding to charge at $S_k$. The two decision variables can be denoted by 
\begin{align}
b_k\!\in\!\{0,1\},~t_k\!\in\!\Re_+,~k\!=\!1,\dots,N,\label{Eq.1}
\end{align}
where $b_k\!=\!1$ if the truck decides to charge at its $k$-th charging station and $0$ otherwise, and $t_k$ denotes the planned charging time of the truck at $S_k$ if $b_k\!=\!1$, with $\Re_+$ representing the set of nonnegative reals. 

In the following, we introduce truck dynamics on its remaining battery and waiting budget, which is built upon the truck's decisions at each charging station along its route.
\subsubsection{Remaining Battery} Let $e_{\text{ini}}$ be the initial battery in a truck at its origin and $e_k$ its remaining battery when it first arrives at its ramp $r_k$, which can be described by
\begin{subequations}
\begin{align}
&e_1=e_{\text{ini}}-\bar{P}\tau_0,\label{Eq.2a}\\
&e_{k+1}=e_k+b_k\Delta{e_k}-\bar{P}\tau_k,\quad k\!=\!1,\dots,N,\label{Eq.2b}
\end{align}
\end{subequations}
where $\bar{P}$ is the truck's battery consumption per travel time unit and $\Delta{e}_k$ denotes the increased battery charged at the station $S_k$. To ensure that the remaining battery of a truck when it arrives at its ramp $r_k$ is sufficient for reaching $S_k$, it requires that
\begin{subequations}
\begin{align}
&e_k\geq{e_s}+\bar{P}d_k, \quad k\!=\!1,\dots,N,\label{Eq.3a}\\
&e_{N+1}\geq{e_s},\label{Eq.3b}
\end{align}
\end{subequations}
where $e_s$ is a constant margin for safe operation. In this paper, the charging process of each truck is approximately modeled by a linear model, as adopted in \cite{liu2021optimal}, as the form of
\begin{align}
\Delta{e_k}=t_k\min\big\{P_k,P_{\max}\big\},\quad k\!=\!1,\dots,N,\label{Eq.4}
\end{align}
where $P_k$ denotes the charging power provided by $S_k$ while $P_{\max}$ is the maximum charging power acceptable by the truck's battery. Restricted by the battery capacity of the truck, $\Delta{e_k}$ is confined by  
\begin{align}
{0}\leq\Delta{e_k}\leq{e_f}\!-\!\big(e_k\!-\!\bar{P}d_k\big),\quad k\!=\!1,\dots,N,\label{Eq.5}
\end{align}
where $e_f$ is the full battery of the truck.
\subsubsection{Remaining Waiting Budget} Trucks usually have delivery deadlines to respect in order to complete delivery missions on time. Apart from the necessary travel time on routes, denoted by $\sum_{k=0}^N\!\tau_k$, the maximum extra time allowed for the trip delay is known as a truck's waiting budget, denoted as $T_w$. 

Making different charging decisions will result in different detours. Seeing that the occupancy of a charging station is unpredictable with the waiting time needed to have an available charging port being uncertain, one cannot guarantee that every truck respects its delivery deadline subject to limited charging resources at stations. In this work, we account for the extra travel and waiting time as additional labor costs and impose a large penalty on the truck's total operational cost if it violates its delivery deadline. To this end, the remaining waiting budget of a truck upon arriving at its ramp $r_k$ can be depicted by
\begin{align}
T_{w,k}=T_w-\sum_{h=1}^{k-1}b_h\big(2d_h\!+\!t_h\!+\!w_h\big),\label{Eq.6}
\end{align}
where $w_h\!\in\!\Re_{+}$ denotes the real waiting time used by the truck to acquire a charging port at its charging station $S_h$.  

\subsection{Distributed Optimal Charging Problem}
To proceed, we denote by $\kappa$ the monetary loss per extra travel time due to detour or waiting for charging, and by $\epsilon_k$ the electricity price per charging time at the station $S_k$.

Based on our proposed two-layer coordination framework, every truck that arrives at its ramp $r_h$ with $h\!=\!k,\dots, N$,  communicates with the charging station $S_k$, obtain the least waiting time it needs to have a port, denoted by $\tilde{w}_k$, and resolves the following distributed optimization problem to determine its charging strategy.
\begin{align}
\min_{\{(b_h,t_h)\}_{h=k}^N}&\kappa\Big(b_k\big(2d_k\!+\!t_k\!+\!\tilde{w}_k\big)+\!\sum_{h=k+1}^N\!\!\!b_h\big(2d_h\!+\!t_h\!+\!\hat{w}_h\big)\Big)\nonumber\\&+\sum_{h=k}^N\!\epsilon_h{b_h}{t_h}+\max\big\{-\!\rho{T_{w,k}},0\big\}\label{Eq.7}
\end{align}
\begin{subequations}
    \begin{align}
    \mathrm{s.\,t.}\quad (\ref{Eq.1})-(\ref{Eq.6}),\nonumber
\end{align}
\end{subequations}
where $\rho$ is some big positive constant introduced to add a penalty if the truck fails to catch up to the latest arrival time at its destination. 

\begin{remark}
The problem in (\ref{Eq.7}) is a mixed integer linear program with bilinear constraints, which is hard to address by many standard solvers. We provide in~\cite{bai2023} a standard method to transform the bilinear constraints into linear ones, which can be used to obtain exact solutions to the problem with the drawback of time-consuming, especially for long-haul trips with a lot of candidate charging stations. To meet the requirement of on-board real-time control, a rollout-based near-optimal solution approach is given in~\cite{10147895}.      
\end{remark}
